Revisiting Self-Training for Few-Shot Learning of Language Model

As unlabeled data carry rich task-relevant information, they are proven useful for few-shot learning of language model. The question is how to effectively make use of such data. In this work, we revisit the self-training technique for language model fine-tuning and present a state-of-the-art prompt-based few-shot learner, SFLM. Given two views of a text sample via weak and strong augmentation techniques, SFLM generates a pseudo label on the weakly augmented version. Then, the model predicts the same pseudo label when fine-tuned with the strongly augmented version. This simple approach is shown to outperform other state-of-the-art supervised and semi-supervised counterparts on six sentence classification and six sentence-pair classification benchmarking tasks. In addition, SFLM only relies on a few in-domain unlabeled data. We conduct a comprehensive analysis to demonstrate the robustness of our proposed approach under various settings, including augmentation techniques, model scale, and few-shot knowledge transfer across tasks.

==> ethics.tex <==
\section{Ethical Considerations \& Broader Impact}
\label{sec:ec}
This study conforms to the prevailing ethical guidelines. All datasets used are in the public domain. In addition, our approach contributes to Green AI, which is more environmentally friendly, and computational efficient. Our approach only relies on few labeled and unlabeled data. Compared to previous approaches that fine-tune the language models on tens of thousands of labeled data, our approach consumes considerably less power.

% In addition, we have identified a way that DynaEval can help address the ethical concerns. By explicitly training the framework to discriminate safe dialogues from unsafe ones, it can help detect dialogues containing inappropriate sentences, such as those regarding injustice and discrimination. Such application may be useful in many real-life scenarios where the behaviors of chatbots need to be properly monitored to avoid insensitive and irresponsible comments from the chatbots.

==> table/table5.tex <==
\begin{table*}
% \small
\centering
\begin{tabular}{ll}
\toprule
                   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{SST-2}\\ (acc)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{SST-5}\\ (acc)\end{tabular}}   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{MR}\\ (acc)\end{tabular}}   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{CR}\\ (acc)\end{tabular}}   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{MPQA}\\ (acc)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Subj}\\ (acc)\end{tabular}} \\ \midrule
FT        & \multicolumn{1}{c}{78.3 (3.7)}                                & \multicolumn{1}{c}{36.4 (2.1)}                                                    & \multicolumn{1}{c}{69.5 (4.3)}                                                    & \multicolumn{1}{c}{78.6 (4.3)}                                                    & \multicolumn{1}{c}{69.2 (7.2)}                                                     & \multicolumn{1}{c}{89.6 (0.8)}                                                    \\ 
LM-BFF  & \multicolumn{1}{c}{89.9 (0.5)}   & \multicolumn{1}{c}{45.8 (3.1)} & \multicolumn{1}{c}{84.1 (1.7)}  & \multicolumn{1}{c}{89.5 (0.6)}    & \multicolumn{1}{c}{84.3 (1.1)}  & \multicolumn{1}{c}{88.3 (3.5)}            \\
PET-few$^\spadesuit$                & \multicolumn{1}{c}{89.8 (0.9)}     & \multicolumn{1}{c}{46.7 (0.8)}                                                & \multicolumn{1}{c}{84.2 (1.2)}                                                 & \multicolumn{1}{c}{89.4 (0.7)}                                                & \multicolumn{1}{c}{84.9 (0.9)}                                                & \multicolumn{1}{c}{90.0 (1.7)}  \\
PET-full$^\heartsuit$    & \multicolumn{1}{c}{90.2 (0.8)}    &  \multicolumn{1}{c}{46.0 (1.2)}                               & \multicolumn{1}{c}{85.0 (1.3)}                               & \multicolumn{1}{c}{88.9 (1.0)}                               & \multicolumn{1}{c}{84.1 (1.0)}                               & \multicolumn{1}{c}{91.4 (0.7)} \\ \midrule
SFLM               & \multicolumn{1}{c}{\textbf{91.0} (0.7)}          & \multicolumn{1}{c}{\textbf{47.7} (1.1)}                               & \multicolumn{1}{c}{\textbf{86.6} (0.4)}                               & \multicolumn{1}{c}{\textbf{90.8} (0.6)}                               & \multicolumn{1}{c}{\textbf{86.5} (0.3)}                               & \multicolumn{1}{c}{\textbf{92.4} (0.7)}                                         \\


\bottomrule
\end{tabular}

\caption{\label{dataset-description}
The datasets evaluated in our work, and corresponding prompt.} 
\end{table*}
